Hashing embeddings of optimal dimension, with applications to linear least squares

The aim of this paper is two-fold: firstly, to present subspace embedding properties for $s$-hashing sketching matrices, with $s\geq 1$, that are optimal in the projection dimension $m$ of the sketch, namely, $m=\mathcal{O}(d)$, where $d$ is the dimension of the subspace. A diverse set of results are presented that address the case when the input matrix has sufficiently low coherence (thus removing the $\log^2 d$ factor dependence in $m$, in the low-coherence result of Bourgain et al (2015) at the expense of a smaller coherence requirement); how this coherence changes with the number $s$ of column nonzeros (allowing a scaling of $\sqrt{s}$ of the coherence bound), or is reduced through suitable transformations (when considering hashed -- instead of subsampled -- coherence reducing transformations such as randomised Hadamard). Secondly, we apply these general hashing sketching results to the special case of Linear Least Squares (LLS), and develop Ski-LLS, a generic software package for these problems, that builds upon and improves the Blendenpik solver on dense input and the (sequential) LSRN performance on sparse problems. In addition to the hashing sketching improvements, we add suitable linear algebra tools for rank-deficient and for sparse problems that lead Ski-LLS to outperform not only sketching-based routines on randomly generated input, but also state of the art direct solver SPQR and iterative code HSL on certain subsets of the sparse Florida matrix collection; namely, on least squares problems that are significantly overdetermined, or moderately sparse, or difficult.

==> tex_Paper_final/Florida_complete_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\begin{longtable}{|l|l|l|l|l|l|l|l|}
\hline
mat_name              & solver & nrow     & ncolumn & nnz      & iter  & time       & residual    \\ \hline
\endfirsthead
%
\multicolumn{8}{c}%
{{\bfseries Table \thetable\ continued from previous page}} \\
\endhead
%
12month1          & Ls_hsl      & 872622   & 12471   & 22624727 & 1286  & 258.417    & 679.323     \\ \hline
Chem97Zt          & Ls_hsl      & 31022    & 2541    & 62044    & 10000 & 5.032      & 6.87166e-13 \\ \hline
D6-6              & Ls_hsl      & 120576   & 23740   & 146880   & 2     & 0.242      & 339.329     \\ \hline
Delor295K         & Ls_hsl      & 1823928  & 295734  & 2401323  & 1     & 4.603      & 1350.53     \\ \hline
Delor338K         & Ls_hsl      & 887058   & 343236  & 4211599  & 215   & 13.258     & 865.227     \\ \hline
Delor64K          & Ls_hsl      & 1785345  & 64719   & 652140   & 1     & 0.848      & 1336.17     \\ \hline
ESOC              & Ls_hsl      & 327062   & 37830   & 6019939  & 10000 & 464.42     & 17.6288     \\ \hline
EternityII_A      & Ls_hsl      & 150638   & 7362    & 782087   & 529   & 4.807      & 2.85067e-13 \\ \hline
EternityII_E      & Ls_hsl      & 262144   & 11077   & 1503732  & 771   & 13.28      & 4.56254e-13 \\ \hline
EternityII_Etilde & Ls_hsl      & 204304   & 10054   & 1170516  & 1334  & 12.975     & 5.78834e-13 \\ \hline
Franz11           & Ls_hsl      & 47104    & 30144   & 329728   & 83    & 0.879      & 7.5299e-14  \\ \hline
GL7d13            & Ls_hsl      & 47271    & 8899    & 356232   & 19    & 0.222      & 194.072     \\ \hline
GL7d14            & Ls_hsl      & 171375   & 47271   & 1831183  & 23    & 3.052      & 351.082     \\ \hline
GL7d15            & Ls_hsl      & 460261   & 171375  & 6080381  & 32    & 14.104     & 548.477     \\ \hline
GL7d16            & Ls_hsl      & 955128   & 460261  & 14488881 & 22    & 48.236     & 748.754     \\ \hline
GL7d17            & Ls_hsl      & 1548650  & 955128  & 25978098 & 23    & 97.673     & 898.97      \\ \hline
GL7d21            & Ls_hsl      & 1437547  & 822922  & 18174775 & 22    & 115.533    & 1002.88     \\ \hline
GL7d22            & Ls_hsl      & 822922   & 349443  & 8251000  & 16    & 26.668     & 789.409     \\ \hline
GL7d23            & Ls_hsl      & 349443   & 105054  & 2695430  & 16    & 3.466      & 535.686     \\ \hline
GL7d24            & Ls_hsl      & 105054   & 21074   & 593892   & 12    & 0.435      & 302.602     \\ \hline
GL7d25            & Ls_hsl      & 21074    & 2798    & 81671    & 12    & 0.053      & 139.096     \\ \hline
Hardesty2         & Ls_hsl      & 929901   & 303645  & 4020731  & 592   & 24.589     & 550.541     \\ \hline
IG5-17            & Ls_hsl      & 30162    & 27944   & 1035008  & 3315  & 28.434     & 91.0391     \\ \hline
IMDB              & Ls_hsl      & 896308   & 428440  & 3782463  & 3315  & 9999       & 9999        \\ \hline
Kemelmacher       & Ls_hsl      & 28452    & 9693    & 100875   & 108   & 0.236      & 113.943     \\ \hline
LargeRegFile      & Ls_hsl      & 2111154  & 801374  & 4944201  & 34    & 12.038     & 444.218     \\ \hline
Maragal_6         & Ls_hsl      & 21255    & 10152   & 537694   & 368   & 14.513     & 94.0062     \\ \hline
Maragal_7         & Ls_hsl      & 46845    & 26564   & 1200537  & 444   & 12.774     & 133.127     \\ \hline
Maragal_8         & Ls_hsl      & 75077    & 33212   & 1308415  & 8453  & 80.994     & 267.052     \\ \hline
NotreDame_actors  & Ls_hsl      & 392400   & 127823  & 1470404  & 7052  & 217.356    & 315.828     \\ \hline
Rucci1            & Ls_hsl      & 1977885  & 109900  & 7791168  & 4272  & 324.326    & 728.373     \\ \hline
TF17              & Ls_hsl      & 48630    & 38132   & 586218   & 4442  & 27.358     & 1.00002     \\ \hline
TF18              & Ls_hsl      & 123867   & 95368   & 1597545  & 10000 & 153.86     & 0.00502214  \\ \hline
TF19              & Ls_hsl      & 317955   & 241029  & 4370721  & 10000 & 555.568    & 0.00715862  \\ \hline
abtaha2           & Ls_hsl      & 37932    & 331     & 137228   & 30    & 0.121      & 139.627     \\ \hline
bibd_17_8         & Ls_hsl      & 24310    & 136     & 680680   & 55    & 0.578      & 4.17609e-14 \\ \hline
bibd_18_9         & Ls_hsl      & 48620    & 153     & 1750320  & 63    & 1.336      & 5.40115e-14 \\ \hline
bibd_19_9         & Ls_hsl      & 92378    & 171     & 3325608  & 60    & 2.973      & 6.46607e-14 \\ \hline
bibd_20_10        & Ls_hsl      & 184756   & 190     & 8314020  & 82    & 7.677      & 1.08516e-13 \\ \hline
bibd_22_8         & Ls_hsl      & 319770   & 231     & 8953560  & 60    & 16.22      & 1.91586e-13 \\ \hline
bibd_81_3         & Ls_hsl      & 85320    & 3240    & 255960   & 32    & 0.168      & 5.98326e-14 \\ \hline
car4              & Ls_hsl      & 33052    & 16384   & 63724    & 3     & 0.066      & 181.585     \\ \hline
cat_ears_4_4      & Ls_hsl      & 44448    & 19020   & 132888   & 28    & 0.677      & 5.20908     \\ \hline
ch7-8-b3          & Ls_hsl      & 58800    & 11760   & 235200   & 11    & 2.168      & 87.8878     \\ \hline
ch7-8-b4          & Ls_hsl      & 141120   & 58800   & 705600   & 44    & 6.674      & 1.36727e-13 \\ \hline
ch7-9-b3          & Ls_hsl      & 105840   & 17640   & 423360   & 10    & 3.649      & 117.943     \\ \hline
ch7-9-b4          & Ls_hsl      & 317520   & 105840  & 1587600  & 48    & 20.756     & 1.85472e-13 \\ \hline
ch7-9-b5          & Ls_hsl      & 423360   & 317520  & 2540160  & 18    & 6.514      & 136.59      \\ \hline
ch8-8-b3          & Ls_hsl      & 117600   & 18816   & 470400   & 16    & 3.88       & 127.009     \\ \hline
ch8-8-b4          & Ls_hsl      & 376320   & 117600  & 1881600  & 43    & 25.357     & 1.78018e-13 \\ \hline
ch8-8-b5          & Ls_hsl      & 564480   & 376320  & 3386880  & 13    & 22.005     & 177.757     \\ \hline
cis-n4c6-b13      & Ls_hsl      & 25605    & 6300    & 88200    & 0     & 0.674      & 160.016     \\ \hline
cis-n4c6-b4       & Ls_hsl      & 20058    & 5970    & 100290   & 38    & 0.917      & 5.15121e-14 \\ \hline
co9               & Ls_hsl      & 22924    & 10789   & 109651   & 978   & 1.337      & 104.725     \\ \hline
connectus         & Ls_hsl      & 394792   & 512     & 1127525  & 175   & 1.819      & 282.669     \\ \hline
cont11_l          & Ls_hsl      & 1961394  & 1468599 & 5382999  & 1     & 36.435     & 1400.5      \\ \hline
cq9               & Ls_hsl      & 21534    & 9278    & 96653    & 554   & 1.149      & 99.855      \\ \hline
dbic1             & Ls_hsl      & 226317   & 43200   & 1081843  & 201   & 3.548      & 199.883     \\ \hline
dbir1             & Ls_hsl      & 45775    & 18804   & 1077025  & 632   & 4.466      & 167.106     \\ \hline
dbir2             & Ls_hsl      & 45877    & 18906   & 1158159  & 10000 & 62.408     & 167.325     \\ \hline
degme             & Ls_hsl      & 659415   & 185501  & 8127528  & 11    & 6.262      & 346.035     \\ \hline
deltaX            & Ls_hsl      & 68600    & 21961   & 247424   & 511   & 1.805      & 27.6767     \\ \hline
deter3            & Ls_hsl      & 21777    & 7647    & 44547    & 176   & 0.331      & 121.959     \\ \hline
e18               & Ls_hsl      & 38602    & 24617   & 156466   & 128   & 0.658      & 118.332     \\ \hline
flower_7_4        & Ls_hsl      & 67593    & 27693   & 202218   & 22    & 1.05       & 5.72223     \\ \hline
flower_8_4        & Ls_hsl      & 125361   & 55081   & 375266   & 32    & 5.745      & 6.58732     \\ \hline
fome11            & Ls_hsl      & 24460    & 12142   & 71264    & 104   & 0.65       & 78.0266     \\ \hline
fome12            & Ls_hsl      & 48920    & 24284   & 142528   & 106   & 1.235      & 110.346     \\ \hline
fome13            & Ls_hsl      & 97840    & 48568   & 285056   & 105   & 2.47       & 156.053     \\ \hline
fome20            & Ls_hsl      & 108175   & 33874   & 232647   & 50    & 0.966      & 60.4874     \\ \hline
fome21            & Ls_hsl      & 216350   & 67748   & 465294   & 51    & 1.906      & 85.5422     \\ \hline
fxm3_16           & Ls_hsl      & 85575    & 41340   & 392252   & 246   & 1.389      & 115.444     \\ \hline
fxm4_6            & Ls_hsl      & 47185    & 22400   & 265442   & 302   & 0.974      & 95.9425     \\ \hline
graphics          & Ls_hsl      & 29493    & 11822   & 117954   & 30    & 0.307      & 0.000303334 \\ \hline
image_interp      & Ls_hsl      & 240000   & 120000  & 711683   & 546   & 6.77       & 466.585     \\ \hline
karted            & Ls_hsl      & 133115   & 46502   & 1770349  & 16    & 1.978      & 112.839     \\ \hline
kl02              & Ls_hsl      & 36699    & 71      & 212536   & 32    & 0.092      & 1.47481e-13 \\ \hline
landmark          & Ls_hsl      & 71952    & 2704    & 1151232  & 36    & 0.356      & 1.12711e-05 \\ \hline
lp_cre_d          & Ls_hsl      & 73948    & 8926    & 246614   & 1687  & 3.534      & 68.8273     \\ \hline
lp_ken_11         & Ls_hsl      & 21349    & 14694   & 49058    & 12    & 0.225      & 61.7298     \\ \hline
lp_ken_13         & Ls_hsl      & 42659    & 28632   & 97246    & 26    & 2.628      & 100.314     \\ \hline
lp_ken_18         & Ls_hsl      & 154699   & 105127  & 358171   & 35    & 11.288     & 162.388     \\ \hline
lp_nug15          & Ls_hsl      & 22275    & 6330    & 94950    & 51    & 0.451      & 4.14953e-13 \\ \hline
lp_nug20          & Ls_hsl      & 72600    & 15240   & 304800   & 36    & 1.039      & 1.15759e-13 \\ \hline
lp_nug30          & Ls_hsl      & 379350   & 52260   & 1567800  & 53    & 4.44       & 2.42959e-13 \\ \hline
lp_osa_07         & Ls_hsl      & 25067    & 1118    & 144812   & 61    & 0.144      & 3.59315     \\ \hline
lp_osa_14         & Ls_hsl      & 54797    & 2337    & 317097   & 62    & 0.323      & 3.61764     \\ \hline
lp_osa_30         & Ls_hsl      & 104374   & 4350    & 604488   & 66    & 0.672      & 3.6446      \\ \hline
lp_osa_60         & Ls_hsl      & 243246   & 10280   & 1408073  & 63    & 1.778      & 3.65144     \\ \hline
lp_pds_06         & Ls_hsl      & 29351    & 9881    & 63220    & 31    & 0.292      & 21.6355     \\ \hline
lp_pds_10         & Ls_hsl      & 49932    & 16558   & 107605   & 32    & 0.459      & 31.6803     \\ \hline
lp_pds_20         & Ls_hsl      & 108175   & 33874   & 232647   & 50    & 0.974      & 60.4874     \\ \hline
lp_qap15          & Ls_hsl      & 22275    & 6330    & 94950    & 42    & 0.129      & 6.20203e-14 \\ \hline
lp_stocfor3       & Ls_hsl      & 23541    & 16675   & 76473    & 299   & 0.431      & 64.4973     \\ \hline
lpl3              & Ls_hsl      & 33686    & 10828   & 100525   & 6     & 0.127      & 93.2339     \\ \hline
mesh_deform       & Ls_hsl      & 234023   & 9393    & 853829   & 5     & 0.244      & 474.231     \\ \hline
mk12-b3           & Ls_hsl      & 51975    & 13860   & 207900   & 9     & 2.028      & 70.5031     \\ \hline
mk12-b5           & Ls_hsl      & 62370    & 10395   & 62370    & 0     & 0.00600004 & 249.74      \\ \hline
mk13-b5           & Ls_hsl      & 270270   & 135135  & 810810   & 0     & 7.09       & 519.875     \\ \hline
mod2              & Ls_hsl      & 66409    & 34774   & 199810   & 99    & 0.654      & 127.97      \\ \hline
mri1              & Ls_hsl      & 147456   & 65536   & 589824   & 542   & 4.036      & 183.123     \\ \hline
mri2              & Ls_hsl      & 147456   & 63240   & 569160   & 1504  & 14.51      & 250.625     \\ \hline
n4c6-b10          & Ls_hsl      & 186558   & 132402  & 1456422  & 12    & 20.354     & 423.391     \\ \hline
n4c6-b11          & Ls_hsl      & 132402   & 69235   & 830820   & 0     & 9.273      & 363.871     \\ \hline
n4c6-b12          & Ls_hsl      & 69235    & 25605   & 332865   & 11    & 2.952      & 260.254     \\ \hline
n4c6-b13          & Ls_hsl      & 25605    & 6300    & 88200    & 0     & 0.651      & 160.016     \\ \hline
n4c6-b4           & Ls_hsl      & 20058    & 5970    & 100290   & 38    & 0.941      & 5.15121e-14 \\ \hline
n4c6-b5           & Ls_hsl      & 51813    & 20058   & 310878   & 11    & 3.048      & 71.6324     \\ \hline
n4c6-b6           & Ls_hsl      & 104115   & 51813   & 728805   & 41    & 6.467      & 1.10658e-13 \\ \hline
n4c6-b7           & Ls_hsl      & 163215   & 104115  & 1305720  & 12    & 10.662     & 101.471     \\ \hline
n4c6-b8           & Ls_hsl      & 198895   & 163215  & 1790055  & 51    & 11.919     & 1.42276e-13 \\ \hline
nemsemm1          & Ls_hsl      & 75352    & 3945    & 1053986  & 16    & 0.309      & 88.6743     \\ \hline
nemsemm2          & Ls_hsl      & 48878    & 6943    & 182012   & 32    & 0.336      & 84.3523     \\ \hline
nemswrld          & Ls_hsl      & 28550    & 7138    & 192283   & 46    & 0.289      & 57.9903     \\ \hline
nsct              & Ls_hsl      & 37563    & 23003   & 697738   & 2804  & 11.785     & 183.944     \\ \hline
nsct_A_1          & Ls_hsl      & 37461    & 22901   & 678739   & 529   & 3.243      & 183.656     \\ \hline
nsct_A_2          & Ls_hsl      & 37563    & 23003   & 697738   & 2804  & 11.929     & 183.944     \\ \hline
nug08-3rd         & Ls_hsl      & 29856    & 19728   & 148416   & 244   & 0.767      & 2.45241e-13 \\ \hline
nw14              & Ls_hsl      & 123409   & 73      & 904910   & 20    & 0.188      & 38.73       \\ \hline
pds-100           & Ls_hsl      & 514577   & 156243  & 1096002  & 102   & 5.558      & 248.562     \\ \hline
pds-30            & Ls_hsl      & 158489   & 49944   & 340635   & 66    & 1.572      & 91.401      \\ \hline
pds-40            & Ls_hsl      & 217531   & 66844   & 466800   & 82    & 2.251      & 121.537     \\ \hline
pds-50            & Ls_hsl      & 275814   & 83060   & 590833   & 84    & 2.835      & 149.42      \\ \hline
pds-60            & Ls_hsl      & 336421   & 99431   & 719557   & 93    & 3.546      & 174.41      \\ \hline
pds-70            & Ls_hsl      & 390005   & 114944  & 833465   & 96    & 3.977      & 196.084     \\ \hline
pds-80            & Ls_hsl      & 434580   & 129181  & 927826   & 96    & 4.691      & 215.247     \\ \hline
pds-90            & Ls_hsl      & 475448   & 142823  & 1014136  & 99    & 5.293      & 232.456     \\ \hline
pltexpa           & Ls_hsl      & 70364    & 26894   & 143059   & 29    & 0.129      & 154.745     \\ \hline
psse0             & Ls_hsl      & 26722    & 11028   & 102432   & 18    & 0.238      & 162.889     \\ \hline
psse2             & Ls_hsl      & 28634    & 11028   & 115262   & 231   & 0.989      & 165.964     \\ \hline
rail2586          & Ls_hsl      & 923269   & 2586    & 8011362  & 316   & 22.321     & 141.129     \\ \hline
rail4284          & Ls_hsl      & 1096894  & 4284    & 11284032 & 269   & 29.75      & 169.483     \\ \hline
rail507           & Ls_hsl      & 63516    & 507     & 409856   & 64    & 0.206      & 47.6061     \\ \hline
rail516           & Ls_hsl      & 47827    & 516     & 315412   & 122   & 0.351      & 37.7208     \\ \hline
rail582           & Ls_hsl      & 56097    & 582     & 402290   & 87    & 0.413      & 45.5016     \\ \hline
rel7              & Ls_hsl      & 21924    & 1045    & 50636    & 16    & 0.172      & 115.182     \\ \hline
rel8              & Ls_hsl      & 345688   & 12347   & 821839   & 21    & 0.906      & 465.204     \\ \hline
rel9              & Ls_hsl      & 9888048  & 274669  & 23667183 & 25    & 47.646     & 2518.48     \\ \hline
relat7            & Ls_hsl      & 21924    & 1045    & 81355    & 14    & 0.0540001  & 139.489     \\ \hline
relat7b           & Ls_hsl      & 21924    & 1045    & 81355    & 14    & 0.062      & 139.489     \\ \hline
relat8            & Ls_hsl      & 345688   & 12347   & 1334038  & 19    & 1.1        & 565.33      \\ \hline
relat9            & Ls_hsl      & 12360060 & 549336  & 38955420 & 24    & 60.937     & 3457.36     \\ \hline
rlfddd            & Ls_hsl      & 61521    & 4050    & 264627   & 25    & 0.422      & 156.121     \\ \hline
rlfdual           & Ls_hsl      & 74970    & 8052    & 282031   & 25    & 0.294      & 201.289     \\ \hline
rlfprim           & Ls_hsl      & 62716    & 58866   & 320591   & 1221  & 7.308      & 115.816     \\ \hline
route             & Ls_hsl      & 43019    & 20894   & 206782   & 68    & 0.408      & 143.643     \\ \hline
sc205-2r          & Ls_hsl      & 62423    & 35213   & 123239   & 59    & 2.91       & 203.351     \\ \hline
scagr7-2r         & Ls_hsl      & 46679    & 32847   & 120141   & 106   & 5.2        & 113.273     \\ \hline
scfxm1-2b         & Ls_hsl      & 33047    & 19036   & 111052   & 269   & 0.548      & 65.8498     \\ \hline
scfxm1-2r         & Ls_hsl      & 65943    & 37980   & 221388   & 306   & 1.343      & 93.0852     \\ \hline
scrs8-2r          & Ls_hsl      & 27691    & 14364   & 58439    & 739   & 2.09       & 135.376     \\ \hline
scsd8-2b          & Ls_hsl      & 35910    & 5130    & 112770   & 56    & 0.28       & 189.496     \\ \hline
scsd8-2c          & Ls_hsl      & 35910    & 5130    & 112770   & 56    & 0.285      & 189.496     \\ \hline
scsd8-2r          & Ls_hsl      & 60550    & 8650    & 190210   & 23    & 0.499      & 246.066     \\ \hline
sctap1-2b         & Ls_hsl      & 33858    & 15390   & 99454    & 271   & 0.859      & 123.67      \\ \hline
sctap1-2r         & Ls_hsl      & 63426    & 28830   & 186366   & 301   & 2.045      & 169.411     \\ \hline
sgpf5y6           & Ls_hsl      & 312540   & 246077  & 831976   & 165   & 6.397      & 221.222     \\ \hline
shar_te2-b2       & Ls_hsl      & 200200   & 17160   & 600600   & 33    & 0.824      & 1.29453e-13 \\ \hline
sls               & Ls_hsl      & 1748122  & 62729   & 6804304  & 137   & 31.598     & 1.33992e-12 \\ \hline
south31           & Ls_hsl      & 36321    & 18425   & 112398   & 123   & 6.806      & 188.07      \\ \hline
spal_004          & Ls_hsl      & 321696   & 10203   & 46168124 & 123   & 9999       & 9999        \\ \hline
specular          & Ls_hsl      & 477976   & 1600    & 7647616  & 205   & 7.672      & 2.04012e-11 \\ \hline
stat96v1          & Ls_hsl      & 197472   & 5995    & 588798   & 7     & 0.124      & 441.821     \\ \hline
stat96v2          & Ls_hsl      & 957432   & 29089   & 2852184  & 14    & 0.695      & 972.731     \\ \hline
stat96v3          & Ls_hsl      & 1113780  & 33841   & 3317736  & 15    & 0.848      & 1049.16     \\ \hline
stat96v4          & Ls_hsl      & 63076    & 3173    & 491336   & 31    & 0.228      & 120.516     \\ \hline
stat96v5          & Ls_hsl      & 75779    & 2307    & 233921   & 2     & 0.112      & 274.794     \\ \hline
stormG2_1000      & Ls_hsl      & 1377306  & 528185  & 3459881  & 307   & 83.79      & 896.488     \\ \hline
stormg2-125       & Ls_hsl      & 172431   & 66185   & 433256   & 332   & 2.552      & 316.77      \\ \hline
stormg2-27        & Ls_hsl      & 37485    & 14441   & 94274    & 269   & 0.443      & 146.957     \\ \hline
t0331-4l          & Ls_hsl      & 46915    & 664     & 430982   & 134   & 0.407      & 73.3133     \\ \hline
testbig           & Ls_hsl      & 31223    & 17613   & 61639    & 55    & 0.75       & 143.698     \\ \hline
tomographic1      & Ls_hsl      & 73159    & 59498   & 647495   & 10000 & 81.226     & 171.913     \\ \hline
tp-6              & Ls_hsl      & 1014301  & 142752  & 11537419 & 8     & 6.84       & 355.881     \\ \hline
ts-palko          & Ls_hsl      & 47235    & 22002   & 1076903  & 24    & 1.104      & 61.241      \\ \hline
ulevimin          & Ls_hsl      & 46937    & 6590    & 164538   & 181   & 0.621      & 39.235      \\ \hline
us04              & Ls_hsl      & 28016    & 163     & 297538   & 81    & 0.192      & 26.7477     \\ \hline
watson_1          & Ls_hsl      & 386992   & 201155  & 1055093  & 88    & 5.675      & 216.319     \\ \hline
watson_2          & Ls_hsl      & 677224   & 352013  & 1846391  & 102   & 9.328      & 284.901     \\ \hline
wheel_601         & Ls_hsl      & 902103   & 723605  & 2170814  & 53    & 214.326    & 497.509     \\ \hline
world             & Ls_hsl      & 67147    & 34506   & 198883   & 101   & 0.645      & 130.412     \\ \hline
\caption{Complete benchmark data for LS\_HSL on the Florida matrix collection. }
\label{tab:Florida_HSL}\\
\end{longtable}


%----


% Please add the following required packages to your document preamble:
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\begin{longtable}{|l|l|l|l|l|l|l|l|}
\hline
mat_name & solver & nrow & ncolumn & nnz & iter & time & residual \\ \hline
\endfirsthead
%
\multicolumn{8}{c}%
{{\bfseries Table \thetable\ continued from previous page}} \\
\endhead
%
12month1 & LS_SPQR & 872622 & 12471 & 22624727 & 0 & 8.311 & 934.142 \\ \hline
Chem97Zt & LS_SPQR & 31022 & 2541 & 62044 & 0 & 0.069 & 4.69165e-14 \\ \hline
D6-6 & LS_SPQR & 120576 & 23740 & 146880 & 0 & 0.11 & 339.329 \\ \hline
Delor295K & LS_SPQR & 1823928 & 295734 & 2401323 & 0 & 23.321 & 1350.53 \\ \hline
Delor338K & LS_SPQR & 887058 & 343236 & 4211599 & 0 & 21.103 & 865.226 \\ \hline
Delor64K & LS_SPQR & 1785345 & 64719 & 652140 & 0 & 1.241 & 1336.17 \\ \hline
ESOC & LS_SPQR & 327062 & 37830 & 6019939 & 0 & 106.138 & 6.06107e-09 \\ \hline
EternityII_A & LS_SPQR & 150638 & 7362 & 782087 & 0 & 3.184 & 8.43642e-13 \\ \hline
EternityII_E & LS_SPQR & 262144 & 11077 & 1503732 & 0 & 29.171 & 1.4914e-12 \\ \hline
EternityII_Etilde & LS_SPQR & 204304 & 10054 & 1170516 & 0 & 24.977 & 5.76214e-13 \\ \hline
Franz11 & LS_SPQR & 47104 & 30144 & 329728 & 0 & 9999 & 9999 \\ \hline
GL7d13 & LS_SPQR & 47271 & 8899 & 356232 & 0 & 232.447 & 194.075 \\ \hline
GL7d14 & LS_SPQR & 171375 & 47271 & 1831183 & 0 & 3.852 & 413.975 \\ \hline
GL7d15 & LS_SPQR & 460261 & 171375 & 6080381 & 0 & 39.589 & 678.425 \\ \hline
GL7d16 & LS_SPQR & 955128 & 460261 & 14488881 & 0 & 217.793 & 977.307 \\ \hline
GL7d17 & LS_SPQR & 1548650 & 955128 & 25978098 & 0 & 724.339 & 1244.45 \\ \hline
GL7d21 & LS_SPQR & 1437547 & 822922 & 18174775 & 0 & 9999 & 9999 \\ \hline
GL7d22 & LS_SPQR & 822922 & 349443 & 8251000 & 0 & 238.033 & 907.15 \\ \hline
GL7d23 & LS_SPQR & 349443 & 105054 & 2695430 & 0 & 34.555 & 591.137 \\ \hline
GL7d24 & LS_SPQR & 105054 & 21074 & 593892 & 0 & 1.413 & 324.12 \\ \hline
GL7d25 & LS_SPQR & 21074 & 2798 & 81671 & 0 & 4.47 & 139.096 \\ \hline
Hardesty2 & LS_SPQR & 929901 & 303645 & 4020731 & 0 & 10.497 & 550.541 \\ \hline
IG5-17 & LS_SPQR & 30162 & 27944 & 1035008 & 0 & 175.959 & 91.0385 \\ \hline
IMDB & LS_SPQR & 896308 & 428440 & 3782463 & 0 & 16.348 & 946.735 \\ \hline
Kemelmacher & LS_SPQR & 28452 & 9693 & 100875 & 0 & 0.133 & 113.943 \\ \hline
LargeRegFile & LS_SPQR & 2111154 & 801374 & 4944201 & 0 & 16.472 & 444.218 \\ \hline
Maragal_6 & LS_SPQR & 21255 & 10152 & 537694 & 0 & 94.395 & 94.8322 \\ \hline
Maragal_7 & LS_SPQR & 46845 & 26564 & 1200537 & 0 & 158.954 & 133.699 \\ \hline
Maragal_8 & LS_SPQR & 75077 & 33212 & 1308415 & 0 & 22.3 & 266.019 \\ \hline
NotreDame_actors & LS_SPQR & 392400 & 127823 & 1470404 & 0 & 1.908 & 626.418 \\ \hline
Rucci1 & LS_SPQR & 1977885 & 109900 & 7791168 & 0 & 606.083 & 727.98 \\ \hline
TF17 & LS_SPQR & 48630 & 38132 & 586218 & 0 & 1.424 & 220.522 \\ \hline
TF18 & LS_SPQR & 123867 & 95368 & 1597545 & 0 & 10.436 & 351.947 \\ \hline
TF19 & LS_SPQR & 317955 & 241029 & 4370721 & 0 & 112.419 & 563.875 \\ \hline
abtaha2 & LS_SPQR & 37932 & 331 & 137228 & 0 & 0.496 & 139.627 \\ \hline
bibd_17_8 & LS_SPQR & 24310 & 136 & 680680 & 0 & 0.14 & 8.82895e-13 \\ \hline
bibd_18_9 & LS_SPQR & 48620 & 153 & 1750320 & 0 & 0.369 & 2.58844e-12 \\ \hline
bibd_19_9 & LS_SPQR & 92378 & 171 & 3325608 & 0 & 0.856 & 4.87653e-12 \\ \hline
bibd_20_10 & LS_SPQR & 184756 & 190 & 8314020 & 0 & 2.31 & 7.42777e-12 \\ \hline
bibd_22_8 & LS_SPQR & 319770 & 231 & 8953560 & 0 & 4.122 & 7.78462e-12 \\ \hline
bibd_81_3 & LS_SPQR & 85320 & 3240 & 255960 & 0 & 19.331 & 6.41381e-12 \\ \hline
car4 & LS_SPQR & 33052 & 16384 & 63724 & 0 & 0.0540001 & 181.585 \\ \hline
cat_ears_4_4 & LS_SPQR & 44448 & 19020 & 132888 & 0 & 42.145 & 5.20908 \\ \hline
ch7-8-b3 & LS_SPQR & 58800 & 11760 & 235200 & 0 & 322.896 & 87.8878 \\ \hline
ch7-8-b4 & LS_SPQR & 141120 & 58800 & 705600 & 0 & 1.449 & 375.659 \\ \hline
ch7-9-b3 & LS_SPQR & 105840 & 17640 & 423360 & 0 & 9999 & 9999 \\ \hline
ch7-9-b4 & LS_SPQR & 317520 & 105840 & 1587600 & 0 & 7.463 & 563.489 \\ \hline
ch7-9-b5 & LS_SPQR & 423360 & 317520 & 2540160 & 0 & 41.693 & 650.661 \\ \hline
ch8-8-b3 & LS_SPQR & 117600 & 18816 & 470400 & 0 & 0.497 & 342.929 \\ \hline
ch8-8-b4 & LS_SPQR & 376320 & 117600 & 1881600 & 0 & 9.261 & 613.449 \\ \hline
ch8-8-b5 & LS_SPQR & 564480 & 376320 & 3386880 & 0 & 85.889 & 751.319 \\ \hline
cis-n4c6-b13 & LS_SPQR & 25605 & 6300 & 88200 & 0 & 8.444 & 160.016 \\ \hline
cis-n4c6-b4 & LS_SPQR & 20058 & 5970 & 100290 & 0 & 36.802 & 2.63159e-12 \\ \hline
co9 & LS_SPQR & 22924 & 10789 & 109651 & 0 & 0.173 & 104.725 \\ \hline
connectus & LS_SPQR & 394792 & 512 & 1127525 & 0 & 2.345 & 282.669 \\ \hline
cont11_l & LS_SPQR & 1961394 & 1468599 & 5382999 & 0 & 13.974 & 1400.5 \\ \hline
cq9 & LS_SPQR & 21534 & 9278 & 96653 & 0 & 0.18 & 99.855 \\ \hline
dbic1 & LS_SPQR & 226317 & 43200 & 1081843 & 0 & 2.262 & 199.883 \\ \hline
dbir1 & LS_SPQR & 45775 & 18804 & 1077025 & 0 & 2.387 & 86.8726 \\ \hline
dbir2 & LS_SPQR & 45877 & 18906 & 1158159 & 0 & 2.594 & 84.0801 \\ \hline
degme & LS_SPQR & 659415 & 185501 & 8127528 & 0 & 37.567 & 346.035 \\ \hline
deltaX & LS_SPQR & 68600 & 21961 & 247424 & 0 & 60.669 & 27.6767 \\ \hline
deter3 & LS_SPQR & 21777 & 7647 & 44547 & 0 & 0.14 & 121.959 \\ \hline
e18 & LS_SPQR & 38602 & 24617 & 156466 & 0 & 161.176 & 118.232 \\ \hline
flower_7_4 & LS_SPQR & 67593 & 27693 & 202218 & 0 & 204.355 & 5.72223 \\ \hline
flower_8_4 & LS_SPQR & 125361 & 55081 & 375266 & 0 & 0.325 & 354.064 \\ \hline
fome11 & LS_SPQR & 24460 & 12142 & 71264 & 0 & 1.283 & 78.0266 \\ \hline
fome12 & LS_SPQR & 48920 & 24284 & 142528 & 0 & 2.447 & 110.346 \\ \hline
fome13 & LS_SPQR & 97840 & 48568 & 285056 & 0 & 4.819 & 156.053 \\ \hline
fome20 & LS_SPQR & 108175 & 33874 & 232647 & 0 & 12.046 & 60.4874 \\ \hline
fome21 & LS_SPQR & 216350 & 67748 & 465294 & 0 & 22.578 & 85.5422 \\ \hline
fxm3_16 & LS_SPQR & 85575 & 41340 & 392252 & 0 & 0.173 & 115.444 \\ \hline
fxm4_6 & LS_SPQR & 47185 & 22400 & 265442 & 0 & 0.0829999 & 95.9425 \\ \hline
graphics & LS_SPQR & 29493 & 11822 & 117954 & 0 & 0.0380001 & 0.000303334 \\ \hline
image_interp & LS_SPQR & 240000 & 120000 & 711683 & 0 & 2.134 & 466.585 \\ \hline
karted & LS_SPQR & 133115 & 46502 & 1770349 & 0 & 15.505 & 112.839 \\ \hline
kl02 & LS_SPQR & 36699 & 71 & 212536 & 0 & 0.0780001 & 1.1409e-12 \\ \hline
landmark & LS_SPQR & 71952 & 2704 & 1151232 & 0 & 5.784 & 1.12706e-05 \\ \hline
lp_cre_d & LS_SPQR & 73948 & 8926 & 246614 & 0 & 0.885 & 68.8273 \\ \hline
lp_ken_11 & LS_SPQR & 21349 & 14694 & 49058 & 0 & 0.049 & 61.7298 \\ \hline
lp_ken_13 & LS_SPQR & 42659 & 28632 & 97246 & 0 & 0.096 & 100.314 \\ \hline
lp_ken_18 & LS_SPQR & 154699 & 105127 & 358171 & 0 & 0.583 & 162.388 \\ \hline
lp_nug15 & LS_SPQR & 22275 & 6330 & 94950 & 0 & 16.742 & 1.80953e-12 \\ \hline
lp_nug20 & LS_SPQR & 72600 & 15240 & 304800 & 0 & 314.259 & 6.65794e-12 \\ \hline
lp_nug30 & LS_SPQR & 379350 & 52260 & 1567800 & 0 & 2.535 & 615.914 \\ \hline
lp_osa_07 & LS_SPQR & 25067 & 1118 & 144812 & 0 & 0.0839999 & 3.59315 \\ \hline
lp_osa_14 & LS_SPQR & 54797 & 2337 & 317097 & 0 & 0.179 & 3.61764 \\ \hline
lp_osa_30 & LS_SPQR & 104374 & 4350 & 604488 & 0 & 0.373 & 3.6446 \\ \hline
lp_osa_60 & LS_SPQR & 243246 & 10280 & 1408073 & 0 & 0.969 & 3.65144 \\ \hline
lp_pds_06 & LS_SPQR & 29351 & 9881 & 63220 & 0 & 0.37 & 21.6355 \\ \hline
lp_pds_10 & LS_SPQR & 49932 & 16558 & 107605 & 0 & 1.498 & 31.6803 \\ \hline
lp_pds_20 & LS_SPQR & 108175 & 33874 & 232647 & 0 & 11.979 & 60.4874 \\ \hline
lp_qap15 & LS_SPQR & 22275 & 6330 & 94950 & 0 & 14.546 & 3.37829e-13 \\ \hline
lp_stocfor3 & LS_SPQR & 23541 & 16675 & 76473 & 0 & 0.0320001 & 64.4973 \\ \hline
lpl3 & LS_SPQR & 33686 & 10828 & 100525 & 0 & 0.139 & 93.2339 \\ \hline
mesh_deform & LS_SPQR & 234023 & 9393 & 853829 & 0 & 0.906 & 474.231 \\ \hline
mk12-b3 & LS_SPQR & 51975 & 13860 & 207900 & 0 & 325.052 & 70.5031 \\ \hline
mk12-b5 & LS_SPQR & 62370 & 10395 & 62370 & 0 & 0.023 & 249.74 \\ \hline
mk13-b5 & LS_SPQR & 270270 & 135135 & 810810 & 0 & 4.75 & 519.875 \\ \hline
mod2 & LS_SPQR & 66409 & 34774 & 199810 & 0 & 0.394 & 127.97 \\ \hline
mri1 & LS_SPQR & 147456 & 65536 & 589824 & 0 & 0.889 & 2.14533e+13 \\ \hline
mri2 & LS_SPQR & 147456 & 63240 & 569160 & 0 & 2.019 & 2.30948e+24 \\ \hline
n4c6-b10 & LS_SPQR & 186558 & 132402 & 1456422 & 0 & 24.225 & 431.924 \\ \hline
n4c6-b11 & LS_SPQR & 132402 & 69235 & 830820 & 0 & 7.47 & 363.871 \\ \hline
n4c6-b12 & LS_SPQR & 69235 & 25605 & 332865 & 0 & 9999 & 9999 \\ \hline
n4c6-b13 & LS_SPQR & 25605 & 6300 & 88200 & 0 & 8.399 & 160.016 \\ \hline
n4c6-b4 & LS_SPQR & 20058 & 5970 & 100290 & 0 & 36.641 & 2.63159e-12 \\ \hline
n4c6-b5 & LS_SPQR & 51813 & 20058 & 310878 & 0 & 9999 & 9999 \\ \hline
n4c6-b6 & LS_SPQR & 104115 & 51813 & 728805 & 0 & 2.284 & 322.669 \\ \hline
n4c6-b7 & LS_SPQR & 163215 & 104115 & 1305720 & 0 & 12.62 & 403.999 \\ \hline
n4c6-b8 & LS_SPQR & 198895 & 163215 & 1790055 & 0 & 38.979 & 445.976 \\ \hline
nemsemm1 & LS_SPQR & 75352 & 3945 & 1053986 & 0 & 0.292 & 88.6743 \\ \hline
nemsemm2 & LS_SPQR & 48878 & 6943 & 182012 & 0 & 0.0580001 & 84.3523 \\ \hline
nemswrld & LS_SPQR & 28550 & 7138 & 192283 & 0 & 0.391 & 57.9903 \\ \hline
nsct & LS_SPQR & 37563 & 23003 & 697738 & 0 & 5.14 & 73.7934 \\ \hline
nsct_A_1 & LS_SPQR & 37461 & 22901 & 678739 & 0 & 4.891 & 88.113 \\ \hline
nsct_A_2 & LS_SPQR & 37563 & 23003 & 697738 & 0 & 5.135 & 73.7934 \\ \hline
nug08-3rd & LS_SPQR & 29856 & 19728 & 148416 & 0 & 240.82 & 1.92452e-12 \\ \hline
nw14 & LS_SPQR & 123409 & 73 & 904910 & 0 & 0.183 & 38.73 \\ \hline
pds-100 & LS_SPQR & 514577 & 156243 & 1096002 & 0 & 9999 & 9999 \\ \hline
pds-30 & LS_SPQR & 158489 & 49944 & 340635 & 0 & 30.488 & 91.401 \\ \hline
pds-40 & LS_SPQR & 217531 & 66844 & 466800 & 0 & 73.314 & 121.537 \\ \hline
pds-50 & LS_SPQR & 275814 & 83060 & 590833 & 0 & 125.797 & 149.42 \\ \hline
pds-60 & LS_SPQR & 336421 & 99431 & 719557 & 0 & 205.663 & 174.41 \\ \hline
pds-70 & LS_SPQR & 390005 & 114944 & 833465 & 0 & 357.429 & 196.084 \\ \hline
pds-80 & LS_SPQR & 434580 & 129181 & 927826 & 0 & 478.052 & 215.247 \\ \hline
pds-90 & LS_SPQR & 475448 & 142823 & 1014136 & 0 & 648.818 & 232.456 \\ \hline
pltexpa & LS_SPQR & 70364 & 26894 & 143059 & 0 & 0.421 & 154.745 \\ \hline
psse0 & LS_SPQR & 26722 & 11028 & 102432 & 0 & 0.029 & 162.889 \\ \hline
psse2 & LS_SPQR & 28634 & 11028 & 115262 & 0 & 0.0339999 & 165.964 \\ \hline
rail2586 & LS_SPQR & 923269 & 2586 & 8011362 & 0 & 721.748 & 141.129 \\ \hline
rail4284 & LS_SPQR & 1096894 & 4284 & 11284032 & 0 & 2.155 & 1047.33 \\ \hline
rail507 & LS_SPQR & 63516 & 507 & 409856 & 0 & 1.231 & 47.6061 \\ \hline
rail516 & LS_SPQR & 47827 & 516 & 315412 & 0 & 0.55 & 37.7208 \\ \hline
rail582 & LS_SPQR & 56097 & 582 & 402290 & 0 & 0.647 & 45.5016 \\ \hline
rel7 & LS_SPQR & 21924 & 1045 & 50636 & 0 & 0.425 & 115.182 \\ \hline
rel8 & LS_SPQR & 345688 & 12347 & 821839 & 0 & 0.506 & 587.952 \\ \hline
rel9 & LS_SPQR & 9888048 & 274669 & 23667183 & 0 & 79.283 & 3144.53 \\ \hline
relat7 & LS_SPQR & 21924 & 1045 & 81355 & 0 & 0.58 & 139.489 \\ \hline
relat7b & LS_SPQR & 21924 & 1045 & 81355 & 0 & 0.596 & 139.489 \\ \hline
relat8 & LS_SPQR & 345688 & 12347 & 1334038 & 0 & 0.87 & 587.952 \\ \hline
relat9 & LS_SPQR & 12360060 & 549336 & 38955420 & 0 & 111.78 & 3515.69 \\ \hline
rlfddd & LS_SPQR & 61521 & 4050 & 264627 & 0 & 0.815 & 156.121 \\ \hline
rlfdual & LS_SPQR & 74970 & 8052 & 282031 & 0 & 2.626 & 201.289 \\ \hline
rlfprim & LS_SPQR & 62716 & 58866 & 320591 & 0 & 84.779 & 115.816 \\ \hline
route & LS_SPQR & 43019 & 20894 & 206782 & 0 & 0.384 & 143.643 \\ \hline
sc205-2r & LS_SPQR & 62423 & 35213 & 123239 & 0 & 8.757 & 203.351 \\ \hline
scagr7-2r & LS_SPQR & 46679 & 32847 & 120141 & 0 & 3.659 & 113.206 \\ \hline
scfxm1-2b & LS_SPQR & 33047 & 19036 & 111052 & 0 & 0.0880001 & 65.8498 \\ \hline
scfxm1-2r & LS_SPQR & 65943 & 37980 & 221388 & 0 & 0.308 & 93.0852 \\ \hline
scrs8-2r & LS_SPQR & 27691 & 14364 & 58439 & 0 & 14.363 & 135.374 \\ \hline
scsd8-2b & LS_SPQR & 35910 & 5130 & 112770 & 0 & 1.29 & 189.496 \\ \hline
scsd8-2c & LS_SPQR & 35910 & 5130 & 112770 & 0 & 1.314 & 189.496 \\ \hline
scsd8-2r & LS_SPQR & 60550 & 8650 & 190210 & 0 & 5.608 & 246.066 \\ \hline
sctap1-2b & LS_SPQR & 33858 & 15390 & 99454 & 0 & 4.317 & 123.67 \\ \hline
sctap1-2r & LS_SPQR & 63426 & 28830 & 186366 & 0 & 25.56 & 169.411 \\ \hline
sgpf5y6 & LS_SPQR & 312540 & 246077 & 831976 & 0 & 1.228 & 221.222 \\ \hline
shar_te2-b2 & LS_SPQR & 200200 & 17160 & 600600 & 0 & 9999 & 9999 \\ \hline
sls & LS_SPQR & 1748122 & 62729 & 6804304 & 0 & 16.547 & 1322.17 \\ \hline
south31 & LS_SPQR & 36321 & 18425 & 112398 & 0 & 189.188 & 188.07 \\ \hline
spal_004 & LS_SPQR & 321696 & 10203 & 46168124 & 0 & 7.39 & 567.183 \\ \hline
specular & LS_SPQR & 477976 & 1600 & 7647616 & 0 & 2.324 & 4.07326e-09 \\ \hline
stat96v1 & LS_SPQR & 197472 & 5995 & 588798 & 0 & 0.315 & 441.821 \\ \hline
stat96v2 & LS_SPQR & 957432 & 29089 & 2852184 & 0 & 1.693 & 972.731 \\ \hline
stat96v3 & LS_SPQR & 1113780 & 33841 & 3317736 & 0 & 2.026 & 1049.16 \\ \hline
stat96v4 & LS_SPQR & 63076 & 3173 & 491336 & 0 & 0.119 & 120.516 \\ \hline
stat96v5 & LS_SPQR & 75779 & 2307 & 233921 & 0 & 1.117 & 274.794 \\ \hline
stormG2_1000 & LS_SPQR & 1377306 & 528185 & 3459881 & 0 & 1.593 & 1173.59 \\ \hline
stormg2-125 & LS_SPQR & 172431 & 66185 & 433256 & 0 & 7.276 & 316.765 \\ \hline
stormg2-27 & LS_SPQR & 37485 & 14441 & 94274 & 0 & 0.163 & 146.957 \\ \hline
t0331-4l & LS_SPQR & 46915 & 664 & 430982 & 0 & 1.483 & 73.3133 \\ \hline
testbig & LS_SPQR & 31223 & 17613 & 61639 & 0 & 1.253 & 143.698 \\ \hline
tomographic1 & LS_SPQR & 73159 & 59498 & 647495 & 0 & 153.268 & 1.0841e+11 \\ \hline
tp-6 & LS_SPQR & 1014301 & 142752 & 11537419 & 0 & 17.847 & 355.881 \\ \hline
ts-palko & LS_SPQR & 47235 & 22002 & 1076903 & 0 & 3.893 & 61.241 \\ \hline
ulevimin & LS_SPQR & 46937 & 6590 & 164538 & 0 & 0.134 & 39.235 \\ \hline
us04 & LS_SPQR & 28016 & 163 & 297538 & 0 & 0.134 & 26.7477 \\ \hline
watson_1 & LS_SPQR & 386992 & 201155 & 1055093 & 0 & 0.651 & 216.319 \\ \hline
watson_2 & LS_SPQR & 677224 & 352013 & 1846391 & 0 & 1.165 & 284.901 \\ \hline
wheel_601 & LS_SPQR & 902103 & 723605 & 2170814 & 0 & 15.671 & 949.791 \\ \hline
world & LS_SPQR & 67147 & 34506 & 198883 & 0 & 0.413 & 130.412 \\ \hline
\caption{Complete benchmark data for LS\_SPQR on the Florida matrix collection. }
\label{tab:Florida_SPQR}\\
\end{longtable}

%-----

% Please add the following required packages to your document preamble:
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\begin{longtable}{|l|l|l|l|l|l|l|l|}
\hline
mat_name & solver & nrow & ncolumn & nnz & iter & time & residual \\ \hline
\endfirsthead
%
\multicolumn{8}{c}%
{{\bfseries Table \thetable\ continued from previous page}} \\
\endhead
%
12month1 & Ls_qr & 872622 & 12471 & 22624727 & 64 & 211.194 & 679.321 \\ \hline
Chem97Zt & Ls_qr & 31022 & 2541 & 62044 & 0 & 1.202 & 4.24353e-13 \\ \hline
D6-6 & Ls_qr & 120576 & 23740 & 146880 & 30 & 669.675 & 339.329 \\ \hline
Delor295K & Ls_qr & 1823928 & 295734 & 2401323 & 30 & 9999 & 9999 \\ \hline
Delor338K & Ls_qr & 887058 & 343236 & 4211599 & 30 & 9999 & 9999 \\ \hline
Delor64K & Ls_qr & 1785345 & 64719 & 652140 & 30 & 9999 & 9999 \\ \hline
ESOC & Ls_qr & 327062 & 37830 & 6019939 & 30 & 9999 & 9999 \\ \hline
EternityII_A & Ls_qr & 150638 & 7362 & 782087 & 0 & 40.307 & 1.00903e-12 \\ \hline
EternityII_E & Ls_qr & 262144 & 11077 & 1503732 & 0 & 134.5 & 1.43253e-12 \\ \hline
EternityII_Etilde & Ls_qr & 204304 & 10054 & 1170516 & 0 & 100.316 & 1.25993e-12 \\ \hline
Franz11 & Ls_qr & 47104 & 30144 & 329728 & 0 & 9999 & 9999 \\ \hline
GL7d13 & Ls_qr & 47271 & 8899 & 356232 & 49 & 69.974 & 194.072 \\ \hline
GL7d14 & Ls_qr & 171375 & 47271 & 1831183 & 49 & 9999 & 9999 \\ \hline
GL7d15 & Ls_qr & 460261 & 171375 & 6080381 & 49 & 9999 & 9999 \\ \hline
GL7d16 & Ls_qr & 955128 & 460261 & 14488881 & 49 & 9999 & 9999 \\ \hline
GL7d17 & Ls_qr & 1548650 & 955128 & 25978098 & 49 & 9999 & 9999 \\ \hline
GL7d21 & Ls_qr & 1437547 & 822922 & 18174775 & 49 & 9999 & 9999 \\ \hline
GL7d22 & Ls_qr & 822922 & 349443 & 8251000 & 49 & 9999 & 9999 \\ \hline
GL7d23 & Ls_qr & 349443 & 105054 & 2695430 & 49 & 9999 & 9999 \\ \hline
GL7d24 & Ls_qr & 105054 & 21074 & 593892 & 49 & 9999 & 9999 \\ \hline
GL7d25 & Ls_qr & 21074 & 2798 & 81671 & 49 & 2.769 & 139.096 \\ \hline
Hardesty2 & Ls_qr & 929901 & 303645 & 4020731 & 49 & 9999 & 9999 \\ \hline
IG5-17 & Ls_qr & 30162 & 27944 & 1035008 & 35 & 274.927 & 91.0385 \\ \hline
IMDB & Ls_qr & 896308 & 428440 & 3782463 & 35 & 9999 & 9999 \\ \hline
Kemelmacher & Ls_qr & 28452 & 9693 & 100875 & 69 & 73.377 & 113.943 \\ \hline
LargeRegFile & Ls_qr & 2111154 & 801374 & 4944201 & 69 & 9999 & 9999 \\ \hline
Maragal_6 & Ls_qr & 21255 & 10152 & 537694 & 7 & 70.687 & 150.598 \\ \hline
Maragal_7 & Ls_qr & 46845 & 26564 & 1200537 & 7 & 9999 & 9999 \\ \hline
Maragal_8 & Ls_qr & 75077 & 33212 & 1308415 & 2 & 656.433 & 336.926 \\ \hline
NotreDame_actors & Ls_qr & 392400 & 127823 & 1470404 & 2 & 9999 & 9999 \\ \hline
Rucci1 & Ls_qr & 1977885 & 109900 & 7791168 & 2 & 9999 & 9999 \\ \hline
TF17 & Ls_qr & 48630 & 38132 & 586218 & 2 & 9999 & 9999 \\ \hline
TF18 & Ls_qr & 123867 & 95368 & 1597545 & 2 & 9999 & 9999 \\ \hline
TF19 & Ls_qr & 317955 & 241029 & 4370721 & 2 & 9999 & 9999 \\ \hline
abtaha2 & Ls_qr & 37932 & 331 & 137228 & 49 & 0.0780001 & 139.627 \\ \hline
bibd_17_8 & Ls_qr & 24310 & 136 & 680680 & 0 & 0.0110002 & 2.22808e-13 \\ \hline
bibd_18_9 & Ls_qr & 48620 & 153 & 1750320 & 0 & 0.0249999 & 2.86778e-13 \\ \hline
bibd_19_9 & Ls_qr & 92378 & 171 & 3325608 & 0 & 0.046 & 3.88705e-13 \\ \hline
bibd_20_10 & Ls_qr & 184756 & 190 & 8314020 & 0 & 0.109 & 4.99636e-13 \\ \hline
bibd_22_8 & Ls_qr & 319770 & 231 & 8953560 & 0 & 0.145 & 9.22145e-13 \\ \hline
bibd_81_3 & Ls_qr & 85320 & 3240 & 255960 & 0 & 3.696 & 7.05716e-13 \\ \hline
car4 & Ls_qr & 33052 & 16384 & 63724 & 79 & 68.977 & 181.585 \\ \hline
cat_ears_4_4 & Ls_qr & 44448 & 19020 & 132888 & 72 & 401.46 & 5.20908 \\ \hline
ch7-8-b3 & Ls_qr & 58800 & 11760 & 235200 & 50 & 164.016 & 87.8878 \\ \hline
ch7-8-b4 & Ls_qr & 141120 & 58800 & 705600 & 50 & 9999 & 9999 \\ \hline
ch7-9-b3 & Ls_qr & 105840 & 17640 & 423360 & 52 & 525.203 & 117.943 \\ \hline
ch7-9-b4 & Ls_qr & 317520 & 105840 & 1587600 & 52 & 9999 & 9999 \\ \hline
ch7-9-b5 & Ls_qr & 423360 & 317520 & 2540160 & 52 & 9999 & 9999 \\ \hline
ch8-8-b3 & Ls_qr & 117600 & 18816 & 470400 & 52 & 655.985 & 127.009 \\ \hline
ch8-8-b4 & Ls_qr & 376320 & 117600 & 1881600 & 52 & 9999 & 9999 \\ \hline
ch8-8-b5 & Ls_qr & 564480 & 376320 & 3386880 & 52 & 9999 & 9999 \\ \hline
cis-n4c6-b13 & Ls_qr & 25605 & 6300 & 88200 & 46 & 25.069 & 160.016 \\ \hline
cis-n4c6-b4 & Ls_qr & 20058 & 5970 & 100290 & 0 & 20.378 & 1.11621e-11 \\ \hline
co9 & Ls_qr & 22924 & 10789 & 109651 & 84 & 54.19 & 104.725 \\ \hline
connectus & Ls_qr & 394792 & 512 & 1127525 & 42 & 0.486 & 282.669 \\ \hline
cont11_l & Ls_qr & 1961394 & 1468599 & 5382999 & 42 & 9999 & 9999 \\ \hline
cq9 & Ls_qr & 21534 & 9278 & 96653 & 75 & 38.596 & 99.855 \\ \hline
dbic1 & Ls_qr & 226317 & 43200 & 1081843 & 75 & 9999 & 9999 \\ \hline
dbir1 & Ls_qr & 45775 & 18804 & 1077025 & 87 & 195.905 & 87.0373 \\ \hline
dbir2 & Ls_qr & 45877 & 18906 & 1158159 & 90 & 196.716 & 84.1533 \\ \hline
degme & Ls_qr & 659415 & 185501 & 8127528 & 90 & 9999 & 9999 \\ \hline
deltaX & Ls_qr & 68600 & 21961 & 247424 & 77 & 691.93 & 27.6767 \\ \hline
deter3 & Ls_qr & 21777 & 7647 & 44547 & 67 & 27.968 & 121.959 \\ \hline
e18 & Ls_qr & 38602 & 24617 & 156466 & 67 & 9999 & 9999 \\ \hline
flower_7_4 & Ls_qr & 67593 & 27693 & 202218 & 67 & 9999 & 9999 \\ \hline
flower_8_4 & Ls_qr & 125361 & 55081 & 375266 & 67 & 9999 & 9999 \\ \hline
fome11 & Ls_qr & 24460 & 12142 & 71264 & 75 & 89.541 & 78.0266 \\ \hline
fome12 & Ls_qr & 48920 & 24284 & 142528 & 80 & 711.611 & 110.346 \\ \hline
fome13 & Ls_qr & 97840 & 48568 & 285056 & 80 & 9999 & 9999 \\ \hline
fome20 & Ls_qr & 108175 & 33874 & 232647 & 80 & 9999 & 9999 \\ \hline
fome21 & Ls_qr & 216350 & 67748 & 465294 & 80 & 9999 & 9999 \\ \hline
fxm3_16 & Ls_qr & 85575 & 41340 & 392252 & 80 & 9999 & 9999 \\ \hline
fxm4_6 & Ls_qr & 47185 & 22400 & 265442 & 85 & 514.866 & 95.9425 \\ \hline
graphics & Ls_qr & 29493 & 11822 & 117954 & 77 & 90.14 & 0.000303334 \\ \hline
image_interp & Ls_qr & 240000 & 120000 & 711683 & 77 & 9999 & 9999 \\ \hline
karted & Ls_qr & 133115 & 46502 & 1770349 & 77 & 9999 & 9999 \\ \hline
kl02 & Ls_qr & 36699 & 71 & 212536 & 0 & 0.0079999 & 2.21136e-13 \\ \hline
landmark & Ls_qr & 71952 & 2704 & 1151232 & 59 & 3.079 & 1.12706e-05 \\ \hline
lp_cre_d & Ls_qr & 73948 & 8926 & 246614 & 41 & 36.102 & 68.8273 \\ \hline
lp_ken_11 & Ls_qr & 21349 & 14694 & 49058 & 114 & 43.226 & 61.7298 \\ \hline
lp_ken_13 & Ls_qr & 42659 & 28632 & 97246 & 112 & 394.056 & 100.314 \\ \hline
lp_ken_18 & Ls_qr & 154699 & 105127 & 358171 & 112 & 9999 & 9999 \\ \hline
lp_nug15 & Ls_qr & 22275 & 6330 & 94950 & 0 & 23.647 & 5.20909e-12 \\ \hline
lp_nug20 & Ls_qr & 72600 & 15240 & 304800 & 0 & 322.936 & 4.95472e-11 \\ \hline
lp_nug30 & Ls_qr & 379350 & 52260 & 1567800 & 0 & 9999 & 9999 \\ \hline
lp_osa_07 & Ls_qr & 25067 & 1118 & 144812 & 57 & 0.327 & 3.59315 \\ \hline
lp_osa_14 & Ls_qr & 54797 & 2337 & 317097 & 61 & 1.943 & 3.61764 \\ \hline
lp_osa_30 & Ls_qr & 104374 & 4350 & 604488 & 62 & 9.452 & 3.6446 \\ \hline
lp_osa_60 & Ls_qr & 243246 & 10280 & 1408073 & 63 & 109.338 & 3.65144 \\ \hline
lp_pds_06 & Ls_qr & 29351 & 9881 & 63220 & 69 & 43.725 & 21.6355 \\ \hline
lp_pds_10 & Ls_qr & 49932 & 16558 & 107605 & 68 & 197.825 & 31.6803 \\ \hline
lp_pds_20 & Ls_qr & 108175 & 33874 & 232647 & 68 & 9999 & 9999 \\ \hline
lp_qap15 & Ls_qr & 22275 & 6330 & 94950 & 0 & 23.416 & 5.59364e-12 \\ \hline
lp_stocfor3 & Ls_qr & 23541 & 16675 & 76473 & 125 & 142.464 & 64.4973 \\ \hline
lpl3 & Ls_qr & 33686 & 10828 & 100525 & 66 & 72.314 & 93.2339 \\ \hline
mesh_deform & Ls_qr & 234023 & 9393 & 853829 & 64 & 89.026 & 474.231 \\ \hline
mk12-b3 & Ls_qr & 51975 & 13860 & 207900 & 51 & 238.048 & 70.5031 \\ \hline
mk12-b5 & Ls_qr & 62370 & 10395 & 62370 & 63 & 83.425 & 249.74 \\ \hline
mk13-b5 & Ls_qr & 270270 & 135135 & 810810 & 63 & 9999 & 9999 \\ \hline
mod2 & Ls_qr & 66409 & 34774 & 199810 & 63 & 9999 & 9999 \\ \hline
mri1 & Ls_qr & 147456 & 65536 & 589824 & 63 & 9999 & 9999 \\ \hline
mri2 & Ls_qr & 147456 & 63240 & 569160 & 63 & 9999 & 9999 \\ \hline
n4c6-b10 & Ls_qr & 186558 & 132402 & 1456422 & 63 & 9999 & 9999 \\ \hline
n4c6-b11 & Ls_qr & 132402 & 69235 & 830820 & 63 & 9999 & 9999 \\ \hline
n4c6-b12 & Ls_qr & 69235 & 25605 & 332865 & 63 & 9999 & 9999 \\ \hline
n4c6-b13 & Ls_qr & 25605 & 6300 & 88200 & 46 & 24.877 & 160.016 \\ \hline
n4c6-b4 & Ls_qr & 20058 & 5970 & 100290 & 0 & 19.89 & 1.11621e-11 \\ \hline
n4c6-b5 & Ls_qr & 51813 & 20058 & 310878 & 38 & 687.163 & 71.6324 \\ \hline
n4c6-b6 & Ls_qr & 104115 & 51813 & 728805 & 38 & 9999 & 9999 \\ \hline
n4c6-b7 & Ls_qr & 163215 & 104115 & 1305720 & 38 & 9999 & 9999 \\ \hline
n4c6-b8 & Ls_qr & 198895 & 163215 & 1790055 & 38 & 9999 & 9999 \\ \hline
nemsemm1 & Ls_qr & 75352 & 3945 & 1053986 & 62 & 6.628 & 88.6743 \\ \hline
nemsemm2 & Ls_qr & 48878 & 6943 & 182012 & 64 & 27.463 & 84.3523 \\ \hline
nemswrld & Ls_qr & 28550 & 7138 & 192283 & 55 & 19.704 & 57.9903 \\ \hline
nsct & Ls_qr & 37563 & 23003 & 697738 & 93 & 258.451 & 74.0498 \\ \hline
nsct_A_1 & Ls_qr & 37461 & 22901 & 678739 & 90 & 280.346 & 89.8349 \\ \hline
nsct_A_2 & Ls_qr & 37563 & 23003 & 697738 & 93 & 257.79 & 74.0498 \\ \hline
nug08-3rd & Ls_qr & 29856 & 19728 & 148416 & 0 & 455.888 & 1.61216e-11 \\ \hline
nw14 & Ls_qr & 123409 & 73 & 904910 & 35 & 0.258 & 38.73 \\ \hline
pds-100 & Ls_qr & 514577 & 156243 & 1096002 & 35 & 9999 & 9999 \\ \hline
pds-30 & Ls_qr & 158489 & 49944 & 340635 & 35 & 9999 & 9999 \\ \hline
pds-40 & Ls_qr & 217531 & 66844 & 466800 & 35 & 9999 & 9999 \\ \hline
pds-50 & Ls_qr & 275814 & 83060 & 590833 & 35 & 9999 & 9999 \\ \hline
pds-60 & Ls_qr & 336421 & 99431 & 719557 & 35 & 9999 & 9999 \\ \hline
pds-70 & Ls_qr & 390005 & 114944 & 833465 & 35 & 9999 & 9999 \\ \hline
pds-80 & Ls_qr & 434580 & 129181 & 927826 & 35 & 9999 & 9999 \\ \hline
pds-90 & Ls_qr & 475448 & 142823 & 1014136 & 35 & 9999 & 9999 \\ \hline
pltexpa & Ls_qr & 70364 & 26894 & 143059 & 35 & 9999 & 9999 \\ \hline
psse0 & Ls_qr & 26722 & 11028 & 102432 & 72 & 65.119 & 162.889 \\ \hline
psse2 & Ls_qr & 28634 & 11028 & 115262 & 71 & 74.007 & 165.964 \\ \hline
rail2586 & Ls_qr & 923269 & 2586 & 8011362 & 61 & 7.279 & 141.129 \\ \hline
rail4284 & Ls_qr & 1096894 & 4284 & 11284032 & 62 & 18.481 & 169.483 \\ \hline
rail507 & Ls_qr & 63516 & 507 & 409856 & 55 & 0.183 & 47.6061 \\ \hline
rail516 & Ls_qr & 47827 & 516 & 315412 & 53 & 0.135 & 37.7208 \\ \hline
rail582 & Ls_qr & 56097 & 582 & 402290 & 55 & 0.22 & 45.5016 \\ \hline
rel7 & Ls_qr & 21924 & 1045 & 50636 & 54 & 0.283 & 115.182 \\ \hline
rel8 & Ls_qr & 345688 & 12347 & 821839 & 62 & 189.969 & 465.204 \\ \hline
rel9 & Ls_qr & 9888048 & 274669 & 23667183 & 62 & 9999 & 9999 \\ \hline
relat7 & Ls_qr & 21924 & 1045 & 81355 & 55 & 0.276 & 139.489 \\ \hline
relat7b & Ls_qr & 21924 & 1045 & 81355 & 55 & 0.277 & 139.489 \\ \hline
relat8 & Ls_qr & 345688 & 12347 & 1334038 & 62 & 197.787 & 565.33 \\ \hline
relat9 & Ls_qr & 12360060 & 549336 & 38955420 & 62 & 9999 & 9999 \\ \hline
rlfddd & Ls_qr & 61521 & 4050 & 264627 & 62 & 7.612 & 156.121 \\ \hline
rlfdual & Ls_qr & 74970 & 8052 & 282031 & 63 & 52.251 & 201.289 \\ \hline
rlfprim & Ls_qr & 62716 & 58866 & 320591 & 63 & 9999 & 9999 \\ \hline
route & Ls_qr & 43019 & 20894 & 206782 & 63 & 9999 & 9999 \\ \hline
sc205-2r & Ls_qr & 62423 & 35213 & 123239 & 63 & 9999 & 9999 \\ \hline
scagr7-2r & Ls_qr & 46679 & 32847 & 120141 & 63 & 9999 & 9999 \\ \hline
scfxm1-2b & Ls_qr & 33047 & 19036 & 111052 & 99 & 326.36 & 65.8498 \\ \hline
scfxm1-2r & Ls_qr & 65943 & 37980 & 221388 & 99 & 9999 & 9999 \\ \hline
scrs8-2r & Ls_qr & 27691 & 14364 & 58439 & 153 & 136.413 & 135.374 \\ \hline
scsd8-2b & Ls_qr & 35910 & 5130 & 112770 & 63 & 14.269 & 189.496 \\ \hline
scsd8-2c & Ls_qr & 35910 & 5130 & 112770 & 63 & 14.227 & 189.496 \\ \hline
scsd8-2r & Ls_qr & 60550 & 8650 & 190210 & 63 & 61.856 & 246.066 \\ \hline
sctap1-2b & Ls_qr & 33858 & 15390 & 99454 & 101 & 168.033 & 123.67 \\ \hline
sctap1-2r & Ls_qr & 63426 & 28830 & 186366 & 101 & 9999 & 9999 \\ \hline
sgpf5y6 & Ls_qr & 312540 & 246077 & 831976 & 101 & 9999 & 9999 \\ \hline
shar_te2-b2 & Ls_qr & 200200 & 17160 & 600600 & 0 & 483.374 & 4.12481e-12 \\ \hline
sls & Ls_qr & 1748122 & 62729 & 6804304 & 0 & 9999 & 9999 \\ \hline
south31 & Ls_qr & 36321 & 18425 & 112398 & 81 & 251.15 & 188.07 \\ \hline
spal_004 & Ls_qr & 321696 & 10203 & 46168124 & 0 & 116.253 & 1.53511e-12 \\ \hline
specular & Ls_qr & 477976 & 1600 & 7647616 & 0 & 0.898 & 2.3516e-10 \\ \hline
stat96v1 & Ls_qr & 197472 & 5995 & 588798 & 63 & 24.289 & 441.821 \\ \hline
stat96v2 & Ls_qr & 957432 & 29089 & 2852184 & 63 & 9999 & 9999 \\ \hline
stat96v3 & Ls_qr & 1113780 & 33841 & 3317736 & 63 & 9999 & 9999 \\ \hline
stat96v4 & Ls_qr & 63076 & 3173 & 491336 & 61 & 4.629 & 120.516 \\ \hline
stat96v5 & Ls_qr & 75779 & 2307 & 233921 & 60 & 1.766 & 274.794 \\ \hline
stormG2_1000 & Ls_qr & 1377306 & 528185 & 3459881 & 60 & 9999 & 9999 \\ \hline
stormg2-125 & Ls_qr & 172431 & 66185 & 433256 & 60 & 9999 & 9999 \\ \hline
stormg2-27 & Ls_qr & 37485 & 14441 & 94274 & 77 & 144.713 & 146.957 \\ \hline
t0331-4l & Ls_qr & 46915 & 664 & 430982 & 55 & 0.265 & 73.3133 \\ \hline
testbig & Ls_qr & 31223 & 17613 & 61639 & 97 & 199.56 & 143.698 \\ \hline
tomographic1 & Ls_qr & 73159 & 59498 & 647495 & 97 & 9999 & 9999 \\ \hline
tp-6 & Ls_qr & 1014301 & 142752 & 11537419 & 97 & 9999 & 9999 \\ \hline
ts-palko & Ls_qr & 47235 & 22002 & 1076903 & 97 & 9999 & 9999 \\ \hline
ulevimin & Ls_qr & 46937 & 6590 & 164538 & 68 & 21.172 & 39.235 \\ \hline
us04 & Ls_qr & 28016 & 163 & 297538 & 26 & 0.0470002 & 26.7477 \\ \hline
watson_1 & Ls_qr & 386992 & 201155 & 1055093 & 26 & 9999 & 9999 \\ \hline
watson_2 & Ls_qr & 677224 & 352013 & 1846391 & 26 & 9999 & 9999 \\ \hline
wheel_601 & Ls_qr & 902103 & 723605 & 2170814 & 26 & 9999 & 9999 \\ \hline
world & Ls_qr & 67147 & 34506 & 198883 & 26 & 9999 & 9999 \\ \hline
\caption{Complete benchmark data for \solverName{} on the Florida matrix collection. }
\label{tab:Florida_SKiLLS}\\
\end{longtable}

%---

% Please add the following required packages to your document preamble:
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\begin{longtable}{|l|l|l|l|l|l|l|l|}
\hline
mat_name & solver & nrow & ncolumn & nnz & iter & time & residual \\ \hline
\endfirsthead
%
\multicolumn{8}{c}%
{{\bfseries Table \thetable\ continued from previous page}} \\
\endhead
%
12month1 & Ls_lsrn & 872622 & 12471 & 22624727 & 0 & 9999 & 9999 \\ \hline
Chem97Zt & Ls_lsrn & 31022 & 2541 & 62044 & 10000 & 82.734 & 4.46654e-13 \\ \hline
D6-6 & Ls_lsrn & 120576 & 23740 & 146880 & 10000 & 9999 & 9999 \\ \hline
Delor295K & Ls_lsrn & 1823928 & 295734 & 2401323 & 10000 & 9999 & 9999 \\ \hline
Delor338K & Ls_lsrn & 887058 & 343236 & 4211599 & 10000 & 9999 & 9999 \\ \hline
Delor64K & Ls_lsrn & 1785345 & 64719 & 652140 & 10000 & 9999 & 9999 \\ \hline
ESOC & Ls_lsrn & 327062 & 37830 & 6019939 & 10000 & 9999 & 9999 \\ \hline
EternityII_A & Ls_lsrn & 150638 & 7362 & 782087 & 133 & 461.681 & 1.88151e-12 \\ \hline
EternityII_E & Ls_lsrn & 262144 & 11077 & 1503732 & 133 & 9999 & 9999 \\ \hline
EternityII_Etilde & Ls_lsrn & 204304 & 10054 & 1170516 & 133 & 9999 & 9999 \\ \hline
Franz11 & Ls_lsrn & 47104 & 30144 & 329728 & 133 & 9999 & 9999 \\ \hline
GL7d13 & Ls_lsrn & 47271 & 8899 & 356232 & 28 & 741.944 & 194.072 \\ \hline
GL7d14 & Ls_lsrn & 171375 & 47271 & 1831183 & 28 & 9999 & 9999 \\ \hline
GL7d15 & Ls_lsrn & 460261 & 171375 & 6080381 & 28 & 9999 & 9999 \\ \hline
GL7d16 & Ls_lsrn & 955128 & 460261 & 14488881 & 28 & 9999 & 9999 \\ \hline
GL7d17 & Ls_lsrn & 1548650 & 955128 & 25978098 & 28 & 9999 & 9999 \\ \hline
GL7d21 & Ls_lsrn & 1437547 & 822922 & 18174775 & 28 & 9999 & 9999 \\ \hline
GL7d22 & Ls_lsrn & 822922 & 349443 & 8251000 & 28 & 9999 & 9999 \\ \hline
GL7d23 & Ls_lsrn & 349443 & 105054 & 2695430 & 28 & 9999 & 9999 \\ \hline
GL7d24 & Ls_lsrn & 105054 & 21074 & 593892 & 28 & 9999 & 9999 \\ \hline
GL7d25 & Ls_lsrn & 21074 & 2798 & 81671 & 27 & 26.01 & 139.096 \\ \hline
Hardesty2 & Ls_lsrn & 929901 & 303645 & 4020731 & 27 & 9999 & 9999 \\ \hline
IG5-17 & Ls_lsrn & 30162 & 27944 & 1035008 & 27 & 9999 & 9999 \\ \hline
IMDB & Ls_lsrn & 896308 & 428440 & 3782463 & 27 & 9999 & 9999 \\ \hline
Kemelmacher & Ls_lsrn & 28452 & 9693 & 100875 & 27 & 9999 & 9999 \\ \hline
LargeRegFile & Ls_lsrn & 2111154 & 801374 & 4944201 & 27 & 9999 & 9999 \\ \hline
Maragal_6 & Ls_lsrn & 21255 & 10152 & 537694 & 27 & 9999 & 9999 \\ \hline
Maragal_7 & Ls_lsrn & 46845 & 26564 & 1200537 & 27 & 9999 & 9999 \\ \hline
Maragal_8 & Ls_lsrn & 75077 & 33212 & 1308415 & 27 & 9999 & 9999 \\ \hline
NotreDame_actors & Ls_lsrn & 392400 & 127823 & 1470404 & 27 & 9999 & 9999 \\ \hline
Rucci1 & Ls_lsrn & 1977885 & 109900 & 7791168 & 27 & 9999 & 9999 \\ \hline
TF17 & Ls_lsrn & 48630 & 38132 & 586218 & 27 & 9999 & 9999 \\ \hline
TF18 & Ls_lsrn & 123867 & 95368 & 1597545 & 27 & 9999 & 9999 \\ \hline
TF19 & Ls_lsrn & 317955 & 241029 & 4370721 & 27 & 9999 & 9999 \\ \hline
abtaha2 & Ls_lsrn & 37932 & 331 & 137228 & 31 & 0.706 & 139.627 \\ \hline
bibd_17_8 & Ls_lsrn & 24310 & 136 & 680680 & 96 & 0.651 & 1.03773e-13 \\ \hline
bibd_18_9 & Ls_lsrn & 48620 & 153 & 1750320 & 97 & 1.738 & 1.34971e-13 \\ \hline
bibd_19_9 & Ls_lsrn & 92378 & 171 & 3325608 & 99 & 3.41 & 1.9568e-13 \\ \hline
bibd_20_10 & Ls_lsrn & 184756 & 190 & 8314020 & 101 & 8.658 & 3.1855e-13 \\ \hline
bibd_22_8 & Ls_lsrn & 319770 & 231 & 8953560 & 106 & 11.652 & 4.01078e-13 \\ \hline
bibd_81_3 & Ls_lsrn & 85320 & 3240 & 255960 & 132 & 45.055 & 6.45177e-13 \\ \hline
car4 & Ls_lsrn & 33052 & 16384 & 63724 & 132 & 9999 & 9999 \\ \hline
cat_ears_4_4 & Ls_lsrn & 44448 & 19020 & 132888 & 132 & 9999 & 9999 \\ \hline
ch7-8-b3 & Ls_lsrn & 58800 & 11760 & 235200 & 132 & 9999 & 9999 \\ \hline
ch7-8-b4 & Ls_lsrn & 141120 & 58800 & 705600 & 132 & 9999 & 9999 \\ \hline
ch7-9-b3 & Ls_lsrn & 105840 & 17640 & 423360 & 132 & 9999 & 9999 \\ \hline
ch7-9-b4 & Ls_lsrn & 317520 & 105840 & 1587600 & 132 & 9999 & 9999 \\ \hline
ch7-9-b5 & Ls_lsrn & 423360 & 317520 & 2540160 & 132 & 9999 & 9999 \\ \hline
ch8-8-b3 & Ls_lsrn & 117600 & 18816 & 470400 & 132 & 9999 & 9999 \\ \hline
ch8-8-b4 & Ls_lsrn & 376320 & 117600 & 1881600 & 132 & 9999 & 9999 \\ \hline
ch8-8-b5 & Ls_lsrn & 564480 & 376320 & 3386880 & 132 & 9999 & 9999 \\ \hline
cis-n4c6-b13 & Ls_lsrn & 25605 & 6300 & 88200 & 0 & 269.531 & 160.016 \\ \hline
cis-n4c6-b4 & Ls_lsrn & 20058 & 5970 & 100290 & 104 & 228.922 & 3.9943e-13 \\ \hline
co9 & Ls_lsrn & 22924 & 10789 & 109651 & 104 & 9999 & 9999 \\ \hline
connectus & Ls_lsrn & 394792 & 512 & 1127525 & 29 & 4.355 & 282.669 \\ \hline
cont11_l & Ls_lsrn & 1961394 & 1468599 & 5382999 & 29 & 9999 & 9999 \\ \hline
cq9 & Ls_lsrn & 21534 & 9278 & 96653 & 29 & 9999 & 9999 \\ \hline
dbic1 & Ls_lsrn & 226317 & 43200 & 1081843 & 29 & 9999 & 9999 \\ \hline
dbir1 & Ls_lsrn & 45775 & 18804 & 1077025 & 29 & 9999 & 9999 \\ \hline
dbir2 & Ls_lsrn & 45877 & 18906 & 1158159 & 29 & 9999 & 9999 \\ \hline
degme & Ls_lsrn & 659415 & 185501 & 8127528 & 29 & 9999 & 9999 \\ \hline
deltaX & Ls_lsrn & 68600 & 21961 & 247424 & 29 & 9999 & 9999 \\ \hline
deter3 & Ls_lsrn & 21777 & 7647 & 44547 & 33 & 479.687 & 121.959 \\ \hline
e18 & Ls_lsrn & 38602 & 24617 & 156466 & 33 & 9999 & 9999 \\ \hline
flower_7_4 & Ls_lsrn & 67593 & 27693 & 202218 & 33 & 9999 & 9999 \\ \hline
flower_8_4 & Ls_lsrn & 125361 & 55081 & 375266 & 33 & 9999 & 9999 \\ \hline
fome11 & Ls_lsrn & 24460 & 12142 & 71264 & 33 & 9999 & 9999 \\ \hline
fome12 & Ls_lsrn & 48920 & 24284 & 142528 & 33 & 9999 & 9999 \\ \hline
fome13 & Ls_lsrn & 97840 & 48568 & 285056 & 33 & 9999 & 9999 \\ \hline
fome20 & Ls_lsrn & 108175 & 33874 & 232647 & 33 & 9999 & 9999 \\ \hline
fome21 & Ls_lsrn & 216350 & 67748 & 465294 & 33 & 9999 & 9999 \\ \hline
fxm3_16 & Ls_lsrn & 85575 & 41340 & 392252 & 33 & 9999 & 9999 \\ \hline
fxm4_6 & Ls_lsrn & 47185 & 22400 & 265442 & 33 & 9999 & 9999 \\ \hline
graphics & Ls_lsrn & 29493 & 11822 & 117954 & 33 & 9999 & 9999 \\ \hline
image_interp & Ls_lsrn & 240000 & 120000 & 711683 & 33 & 9999 & 9999 \\ \hline
karted & Ls_lsrn & 133115 & 46502 & 1770349 & 33 & 9999 & 9999 \\ \hline
kl02 & Ls_lsrn & 36699 & 71 & 212536 & 70 & 0.212 & 1.06419e-13 \\ \hline
landmark & Ls_lsrn & 71952 & 2704 & 1151232 & 78 & 32.091 & 1.12704e-05 \\ \hline
lp_cre_d & Ls_lsrn & 73948 & 8926 & 246614 & 26 & 710.099 & 68.8273 \\ \hline
lp_ken_11 & Ls_lsrn & 21349 & 14694 & 49058 & 26 & 9999 & 9999 \\ \hline
lp_ken_13 & Ls_lsrn & 42659 & 28632 & 97246 & 26 & 9999 & 9999 \\ \hline
lp_ken_18 & Ls_lsrn & 154699 & 105127 & 358171 & 26 & 9999 & 9999 \\ \hline
lp_nug15 & Ls_lsrn & 22275 & 6330 & 94950 & 116 & 270.484 & 4.26068e-13 \\ \hline
lp_nug20 & Ls_lsrn & 72600 & 15240 & 304800 & 116 & 9999 & 9999 \\ \hline
lp_nug30 & Ls_lsrn & 379350 & 52260 & 1567800 & 116 & 9999 & 9999 \\ \hline
lp_osa_07 & Ls_lsrn & 25067 & 1118 & 144812 & 42 & 2.745 & 3.59315 \\ \hline
lp_osa_14 & Ls_lsrn & 54797 & 2337 & 317097 & 45 & 18.961 & 3.61764 \\ \hline
lp_osa_30 & Ls_lsrn & 104374 & 4350 & 604488 & 46 & 102.511 & 3.6446 \\ \hline
lp_osa_60 & Ls_lsrn & 243246 & 10280 & 1408073 & 46 & 9999 & 9999 \\ \hline
lp_pds_06 & Ls_lsrn & 29351 & 9881 & 63220 & 46 & 9999 & 9999 \\ \hline
lp_pds_10 & Ls_lsrn & 49932 & 16558 & 107605 & 46 & 9999 & 9999 \\ \hline
lp_pds_20 & Ls_lsrn & 108175 & 33874 & 232647 & 46 & 9999 & 9999 \\ \hline
lp_qap15 & Ls_lsrn & 22275 & 6330 & 94950 & 117 & 270.643 & 4.46178e-13 \\ \hline
lp_stocfor3 & Ls_lsrn & 23541 & 16675 & 76473 & 117 & 9999 & 9999 \\ \hline
lpl3 & Ls_lsrn & 33686 & 10828 & 100525 & 117 & 9999 & 9999 \\ \hline
mesh_deform & Ls_lsrn & 234023 & 9393 & 853829 & 117 & 9999 & 9999 \\ \hline
mk12-b3 & Ls_lsrn & 51975 & 13860 & 207900 & 117 & 9999 & 9999 \\ \hline
mk12-b5 & Ls_lsrn & 62370 & 10395 & 62370 & 117 & 9999 & 9999 \\ \hline
mk13-b5 & Ls_lsrn & 270270 & 135135 & 810810 & 117 & 9999 & 9999 \\ \hline
mod2 & Ls_lsrn & 66409 & 34774 & 199810 & 117 & 9999 & 9999 \\ \hline
mri1 & Ls_lsrn & 147456 & 65536 & 589824 & 117 & 9999 & 9999 \\ \hline
mri2 & Ls_lsrn & 147456 & 63240 & 569160 & 117 & 9999 & 9999 \\ \hline
n4c6-b10 & Ls_lsrn & 186558 & 132402 & 1456422 & 117 & 9999 & 9999 \\ \hline
n4c6-b11 & Ls_lsrn & 132402 & 69235 & 830820 & 117 & 9999 & 9999 \\ \hline
n4c6-b12 & Ls_lsrn & 69235 & 25605 & 332865 & 117 & 9999 & 9999 \\ \hline
n4c6-b13 & Ls_lsrn & 25605 & 6300 & 88200 & 0 & 326.563 & 160.016 \\ \hline
n4c6-b4 & Ls_lsrn & 20058 & 5970 & 100290 & 104 & 232.71 & 4.05413e-13 \\ \hline
n4c6-b5 & Ls_lsrn & 51813 & 20058 & 310878 & 104 & 9999 & 9999 \\ \hline
n4c6-b6 & Ls_lsrn & 104115 & 51813 & 728805 & 104 & 9999 & 9999 \\ \hline
n4c6-b7 & Ls_lsrn & 163215 & 104115 & 1305720 & 104 & 9999 & 9999 \\ \hline
n4c6-b8 & Ls_lsrn & 198895 & 163215 & 1790055 & 104 & 9999 & 9999 \\ \hline
nemsemm1 & Ls_lsrn & 75352 & 3945 & 1053986 & 37 & 80.693 & 88.6743 \\ \hline
nemsemm2 & Ls_lsrn & 48878 & 6943 & 182012 & 36 & 361.098 & 84.3523 \\ \hline
nemswrld & Ls_lsrn & 28550 & 7138 & 192283 & 33 & 383.658 & 57.9903 \\ \hline
nsct & Ls_lsrn & 37563 & 23003 & 697738 & 33 & 9999 & 9999 \\ \hline
nsct_A_1 & Ls_lsrn & 37461 & 22901 & 678739 & 33 & 9999 & 9999 \\ \hline
nsct_A_2 & Ls_lsrn & 37563 & 23003 & 697738 & 33 & 9999 & 9999 \\ \hline
nug08-3rd & Ls_lsrn & 29856 & 19728 & 148416 & 33 & 9999 & 9999 \\ \hline
nw14 & Ls_lsrn & 123409 & 73 & 904910 & 31 & 0.536 & 38.73 \\ \hline
pds-100 & Ls_lsrn & 514577 & 156243 & 1096002 & 31 & 9999 & 9999 \\ \hline
pds-30 & Ls_lsrn & 158489 & 49944 & 340635 & 31 & 9999 & 9999 \\ \hline
pds-40 & Ls_lsrn & 217531 & 66844 & 466800 & 31 & 9999 & 9999 \\ \hline
pds-50 & Ls_lsrn & 275814 & 83060 & 590833 & 31 & 9999 & 9999 \\ \hline
pds-60 & Ls_lsrn & 336421 & 99431 & 719557 & 31 & 9999 & 9999 \\ \hline
pds-70 & Ls_lsrn & 390005 & 114944 & 833465 & 31 & 9999 & 9999 \\ \hline
pds-80 & Ls_lsrn & 434580 & 129181 & 927826 & 31 & 9999 & 9999 \\ \hline
pds-90 & Ls_lsrn & 475448 & 142823 & 1014136 & 31 & 9999 & 9999 \\ \hline
pltexpa & Ls_lsrn & 70364 & 26894 & 143059 & 31 & 9999 & 9999 \\ \hline
psse0 & Ls_lsrn & 26722 & 11028 & 102432 & 31 & 9999 & 9999 \\ \hline
psse2 & Ls_lsrn & 28634 & 11028 & 115262 & 31 & 9999 & 9999 \\ \hline
rail2586 & Ls_lsrn & 923269 & 2586 & 8011362 & 38 & 122.842 & 141.129 \\ \hline
rail4284 & Ls_lsrn & 1096894 & 4284 & 11284032 & 38 & 351.9 & 169.483 \\ \hline
rail507 & Ls_lsrn & 63516 & 507 & 409856 & 36 & 1.317 & 47.6061 \\ \hline
rail516 & Ls_lsrn & 47827 & 516 & 315412 & 36 & 1.165 & 37.7208 \\ \hline
rail582 & Ls_lsrn & 56097 & 582 & 402290 & 36 & 1.385 & 45.5016 \\ \hline
rel7 & Ls_lsrn & 21924 & 1045 & 50636 & 31 & 1.924 & 115.182 \\ \hline
rel8 & Ls_lsrn & 345688 & 12347 & 821839 & 31 & 9999 & 9999 \\ \hline
rel9 & Ls_lsrn & 9888048 & 274669 & 23667183 & 31 & 9999 & 9999 \\ \hline
relat7 & Ls_lsrn & 21924 & 1045 & 81355 & 29 & 2.035 & 139.489 \\ \hline
relat7b & Ls_lsrn & 21924 & 1045 & 81355 & 29 & 2.297 & 139.489 \\ \hline
relat8 & Ls_lsrn & 345688 & 12347 & 1334038 & 29 & 9999 & 9999 \\ \hline
relat9 & Ls_lsrn & 12360060 & 549336 & 38955420 & 29 & 9999 & 9999 \\ \hline
rlfddd & Ls_lsrn & 61521 & 4050 & 264627 & 34 & 78.719 & 156.121 \\ \hline
rlfdual & Ls_lsrn & 74970 & 8052 & 282031 & 33 & 560.187 & 201.289 \\ \hline
rlfprim & Ls_lsrn & 62716 & 58866 & 320591 & 33 & 9999 & 9999 \\ \hline
route & Ls_lsrn & 43019 & 20894 & 206782 & 33 & 9999 & 9999 \\ \hline
sc205-2r & Ls_lsrn & 62423 & 35213 & 123239 & 33 & 9999 & 9999 \\ \hline
scagr7-2r & Ls_lsrn & 46679 & 32847 & 120141 & 33 & 9999 & 9999 \\ \hline
scfxm1-2b & Ls_lsrn & 33047 & 19036 & 111052 & 33 & 9999 & 9999 \\ \hline
scfxm1-2r & Ls_lsrn & 65943 & 37980 & 221388 & 33 & 9999 & 9999 \\ \hline
scrs8-2r & Ls_lsrn & 27691 & 14364 & 58439 & 33 & 9999 & 9999 \\ \hline
scsd8-2b & Ls_lsrn & 35910 & 5130 & 112770 & 20 & 152.052 & 189.496 \\ \hline
scsd8-2c & Ls_lsrn & 35910 & 5130 & 112770 & 20 & 152.266 & 189.496 \\ \hline
scsd8-2r & Ls_lsrn & 60550 & 8650 & 190210 & 19 & 684.441 & 246.066 \\ \hline
sctap1-2b & Ls_lsrn & 33858 & 15390 & 99454 & 19 & 9999 & 9999 \\ \hline
sctap1-2r & Ls_lsrn & 63426 & 28830 & 186366 & 19 & 9999 & 9999 \\ \hline
sgpf5y6 & Ls_lsrn & 312540 & 246077 & 831976 & 19 & 9999 & 9999 \\ \hline
shar_te2-b2 & Ls_lsrn & 200200 & 17160 & 600600 & 19 & 9999 & 9999 \\ \hline
sls & Ls_lsrn & 1748122 & 62729 & 6804304 & 19 & 9999 & 9999 \\ \hline
south31 & Ls_lsrn & 36321 & 18425 & 112398 & 19 & 9999 & 9999 \\ \hline
spal_004 & Ls_lsrn & 321696 & 10203 & 46168124 & 19 & 9999 & 9999 \\ \hline
specular & Ls_lsrn & 477976 & 1600 & 7647616 & 100 & 41.171 & 1.91943e-11 \\ \hline
stat96v1 & Ls_lsrn & 197472 & 5995 & 588798 & 28 & 247.988 & 441.821 \\ \hline
stat96v2 & Ls_lsrn & 957432 & 29089 & 2852184 & 28 & 9999 & 9999 \\ \hline
stat96v3 & Ls_lsrn & 1113780 & 33841 & 3317736 & 28 & 9999 & 9999 \\ \hline
stat96v4 & Ls_lsrn & 63076 & 3173 & 491336 & 35 & 42.353 & 120.516 \\ \hline
stat96v5 & Ls_lsrn & 75779 & 2307 & 233921 & 25 & 17.678 & 274.794 \\ \hline
stormG2_1000 & Ls_lsrn & 1377306 & 528185 & 3459881 & 25 & 9999 & 9999 \\ \hline
stormg2-125 & Ls_lsrn & 172431 & 66185 & 433256 & 25 & 9999 & 9999 \\ \hline
stormg2-27 & Ls_lsrn & 37485 & 14441 & 94274 & 25 & 9999 & 9999 \\ \hline
t0331-4l & Ls_lsrn & 46915 & 664 & 430982 & 35 & 1.828 & 73.3133 \\ \hline
testbig & Ls_lsrn & 31223 & 17613 & 61639 & 35 & 9999 & 9999 \\ \hline
tomographic1 & Ls_lsrn & 73159 & 59498 & 647495 & 35 & 9999 & 9999 \\ \hline
tp-6 & Ls_lsrn & 1014301 & 142752 & 11537419 & 35 & 9999 & 9999 \\ \hline
ts-palko & Ls_lsrn & 47235 & 22002 & 1076903 & 35 & 9999 & 9999 \\ \hline
ulevimin & Ls_lsrn & 46937 & 6590 & 164538 & 38 & 311.379 & 39.235 \\ \hline
us04 & Ls_lsrn & 28016 & 163 & 297538 & 23 & 0.317 & 26.7477 \\ \hline
watson_1 & Ls_lsrn & 386992 & 201155 & 1055093 & 23 & 9999 & 9999 \\ \hline
watson_2 & Ls_lsrn & 677224 & 352013 & 1846391 & 23 & 9999 & 9999 \\ \hline
wheel_601 & Ls_lsrn & 902103 & 723605 & 2170814 & 23 & 9999 & 9999 \\ \hline
world & Ls_lsrn & 67147 & 34506 & 198883 & 23 & 9999 & 9999 \\ \hline
\caption{Complete benchmark data for LSRN on the Florida matrix collection. }
\label{tab:Florida_LSRN}\\
\end{longtable}
